Decadal analysis of sea surface temperature patterns, climatology, and anomalies in temperate coastal waters with Landsat-8 TIRS observations

Sea surface temperature (SST) is a fundamental physical parameter characterising the thermal state of sea surface. Due to the intricate thermal interactions between land, sea, and atmosphere, the spatial gradients of SST in coastal waters often appear at finer spatial scales than those in open ocean waters. The Thermal Infrared Sensor (TIRS) onboard Landsat-8, with its 100-meter spatial resolution, offers a unique opportunity to uncover fine-scale coastal SST patterns that would otherwise be overlooked by coarser-resolution thermal sensors. In this study, we first analysed the spatiotemporal patterns of SST in South Australia's temperate coastal waters from 2014 to 2023 by developing an operational approach for SST retrieval from the Landsat-8 TIRS sensor. A buoy was deployed off the coast of Port Lincoln, South Australia, to validate the quality of SST retrievals. Then the daily baseline climatology of SST with 100 m resolution was constructed, which allowed for the detection and analysis of anomalous SST events. Our results suggest the following: (1) the satellite-derived SST data aligned well with the in-situ measured SST values; (2) the semi-enclosed, shallow regions of Upper Spencer Gulf and Upper St Vincent Gulf showed higher temperatures during summer and cooler temperatures during winter than waters closer to the open ocean, resulting in a higher seasonal variation in SST; (3) the near-shore shallow areas in Spencer Gulf and St Vincent Gulf, and regions surrounding Kangaroo Island, were identified to have a higher probability of SST anomalies compared to the rest of the study area; and (4) anomalous SST events were more likely to happen during the warm months than the cool months. We hope these findings would be helpful in supporting the fishing and aquaculture industries in the coastal waters of South Australia.

==> sections/suppliment_1.tex <==
\appendix
\section*{Appendix A. Atmospheric simulations with libRadtran} 
\label{sec:appendix_a}

Following the approach in \cite{vanhellemont2020automated}, three atmospheric simulations were conducted with the radiative transfer software package \emph{libRadtran} \cite{emde2016libradtran}, to derive the atmospheric upwelling and downwelling radiances, $L_u(\lambda)$ and $L_d(\lambda)$, and the transmittance of atmosphere, $\tau(\lambda)$. It is worth noting that, these simulations were conducted under assumed atmospheric parameters for the purpose of solving the radiative transfer equation (Eq. (\ref{eq:radiative})), rather than simulating with the actual atmospheric conditions.

In the first simulation, we assumed the spectral emissivity of water $\varepsilon(\lambda)$ to be 1 for all wavelengths, and the black-body radiance of water $L_s(\lambda)$ to be the spectral radiance of a 290 K black body. We noted the assumed $\varepsilon(\lambda)$ and $L_s(\lambda)$ values as $\varepsilon^{\text{(1)}}(\lambda)$ and $L_s^{\text{(1)}}(\lambda)$, respectively. Under such assumptions, Eq.~(\ref{eq:radiative}) became:
\begin{equation}
\label{eq:sim1}
\begin{aligned}
    L_t^{\text{(1)}}(\lambda) &= \tau(\lambda) \cdot \varepsilon^{\text{(1)}}(\lambda) \cdot L_s^{\text{(1)}}(\lambda) + L_u(\lambda) + \tau(\lambda) \cdot \left(1 - \varepsilon^{\text{(1)}}(\lambda)\right) \cdot L_d(\lambda) \\
    &= \tau(\lambda) \cdot L_s^{\text{(1)}}(\lambda) + L_u(\lambda),
\end{aligned}
\end{equation}
where $L_t^{\text{(1)}}(\lambda)$ is the \emph{libRadtran}-simulated at-sensor radiance under the $\varepsilon^{\text{(1)}}(\lambda)$ and $L_s^{\text{(1)}}(\lambda)$ assumptions. 

In the second simulation, we assumed $\varepsilon(\lambda)$ to be 1 for all wavelengths and $L_s(\lambda)$ to be the spectral radiance of a 300 K black body, noted as $\varepsilon^{\text{(2)}}(\lambda)$ and $L_s^{\text{(2)}}(\lambda)$, respectively, and Eq.~(\ref{eq:radiative}) became:
\begin{equation}
\label{eq:sim2}
\begin{aligned}
    L_t^{\text{(2)}}(\lambda) &= \tau(\lambda) \cdot \varepsilon^{\text{(2)}}(\lambda) \cdot L_s^{\text{(2)}}(\lambda) + L_u(\lambda) + \tau(\lambda) \cdot \left(1 - \varepsilon^{\text{(2)}}(\lambda)\right) \cdot L_d(\lambda) \\
    &= \tau(\lambda) \cdot L_s^{\text{(2)}}(\lambda) + L_u(\lambda),
\end{aligned}
\end{equation}
where $L_t^{\text{(2)}}(\lambda)$ is the corresponding \emph{libRadtran}-simulated at-sensor radiance under the $\varepsilon^{\text{(2)}}(\lambda)$ and $L_s^{\text{(2)}}(\lambda)$ assumptions. By combining Eqs~(\ref{eq:sim1}) and (\ref{eq:sim2}), the transmittance of atmosphere $\tau(\lambda)$ and atmospheric upwelling radiance $L_u(\lambda)$ were derived as:
\begin{equation}
\label{eq:tau}
\tau(\lambda)=\dfrac{L_t^{\text{(2)}}(\lambda)-L_t^{\text{(1)}}(\lambda)}{L_s^{\text{(2)}}(\lambda)-L_s^{\text{(1)}}(\lambda)},
\end{equation}
\begin{equation}
\label{eq:lu}
L_u(\lambda)=L_t^{\text{(1)}}(\lambda)-\dfrac{L_t^{\text{(2)}}(\lambda)-L_t^{\text{(1)}}(\lambda)}{L_s^{\text{(2)}}(\lambda)-L_s^{\text{(1)}}(\lambda)}\cdot L_s^{\text{(1)}}(\lambda).
\end{equation}

In the third simulation, we assumed $\varepsilon(\lambda)$ to be 0.95 and $L_s(\lambda)$ to be 0 (\emph{i.e.}, equivalent to black-body radiance at 0 K), noted as $\varepsilon^{\text{(3)}}(\lambda)$ and $L_s^{\text{(3)}}(\lambda)$, respectively. Then Eq.~(\ref{eq:radiative}) became:
\begin{equation}
\label{eq:sim3}
\begin{aligned}
    L_t^{\text{(3)}}(\lambda) &= \tau(\lambda)\cdot\varepsilon^{\text{(3)}}(\lambda)\cdot L_s^{\text{(3)}}(\lambda) + L_u(\lambda) + \tau(\lambda)\cdot\left[1-\varepsilon^{\text{(3)}}(\lambda)\right]\cdot L_d(\lambda) \\& = L_u(\lambda) + \tau(\lambda)\cdot\left[1-\varepsilon^{\text{(3)}}(\lambda)\right]\cdot L_d(\lambda),
\end{aligned}
\end{equation}
where $L_t^{\text{(3)}}(\lambda)$ is the corresponding \emph{libRadtran}-simulated at-sensor radiance under the $\varepsilon^{\text{(3)}}(\lambda)$ and $L_s^{\text{(3)}}(\lambda)$ assumptions. Taking into consideration of Eqs~(\ref{eq:tau}), (\ref{eq:lu}), and (\ref{eq:sim3}), the atmospheric downwelling radiance $L_d(\lambda)$ was derived as:
\begin{equation}
\label{eq:ld}
L_d(\lambda) = \dfrac{L_t^{\text{(3)}}(\lambda)-L_t^{\text{(1)}}(\lambda)+\dfrac{L_t^{\text{(2)}}(\lambda)-L_t^{\text{(1)}}(\lambda)}{L_s^{\text{(2)}}(\lambda)-L_s^{\text{(1)}}(\lambda)}\cdot L_s^{\text{(1)}}(\lambda)}{\left[1-\varepsilon^{\text{(3)}}(\lambda)\right]\cdot \dfrac{L_t^{\text{(2)}}(\lambda)-L_t^{\text{(1)}}(\lambda)}{L_s^{\text{(2)}}(\lambda)-L_s^{\text{(1)}}(\lambda)}}.
\end{equation}

It is worth noting that the three \emph{libRadtran} simulations were conducted for the thermal spectral range from 9,000 nm to 14,050 nm at 1 nm spectral sampling interval. Therefore, the derived $\tau(\lambda)$, $L_u(\lambda)$, and $L_d(\lambda)$, based on Eqs~(\ref{eq:tau}), (\ref{eq:lu}), and (\ref{eq:ld}), respectively, were of the same spectral range (9,000--14,050 nm) and interval (1 nm).

==> sections/suppliment_2.tex <==
\section*{Appendix B. Calculation of Atmospheric Parameters} 
\label{sec:appendix_b}

For each cell that covers a spatial span of 0.75 degree longitude by 0.75 degree latitude and a temporal span of 3 hours, the corresponding mean sea level air pressure (single level value at sea surface, in Pa) was retrieved from the CAMS EAC4 data set. It was then converted from the single level air pressure at sea surface, to the vertical profile of air pressure at 60 discretised levels (from sea surface to top of atmosphere), based on the 60-level vertical discretisation model as defined in \cite{74321} and the converting coefficients for each model level as provided in CAMS EAC4:
\begin{equation}
\label{eq:pressure}
p^{(i)}=a^{(i)}+p_0\cdot b^{(i)}
\end{equation}
where $p_0$ is the air pressure at sea surface; $p^{(i)}$ is the air pressure at the $i$th model level; and $a^{(i)}$ and $b^{(i)}$ are the corresponding converting coefficients for that model level. 

Cell-specific retrievals of atmosphere conditions from the CAMS EAC4 data set also included air temperature $T^{(i)}$ (in unit of K), specific humidity $q^{(i)}$ (in unit of kg/kg), ozone concentration $O_3^{(i)}$ (in unit of kg/kg), and nitrogen dioxide concentration $NO_2^{(i)}$ (in unit of kg/kg). All these parameters were provided as vertical profiles at the 60 model levels from sea surface to top of atmosphere, with $i$ ranging from 1 to 60 in their notations.

The altitude of each model level was calculated from the air pressure at sea surface $p_0$ and the vertical profiles of air pressure $p^{(i)}$ and air temperature $T{(i)}$ via the Barometric formula:
\begin{equation}
\label{eq:altitude}
h^{(i)}=-\dfrac{\text{ln}\left(\dfrac{p^{(i)}}{p_0}\right)\cdot R\cdot T^{(i)}}{g\cdot M}+h_0,
\end{equation}
where $h^{(i)}$ is the altitude at the $i$th model level; $h^{(i)}$=0 m is the altitude of sea surface; $g$=9.8067 m/s\textsuperscript{2} is the gravitational acceleration; $R$=8.31446 J/(K·mol) is the universal gas constant; and $M^{(i)}$ is the molar mass of air at the $i$th model level, which was calculated as the combination of molar mass of dry air and water vapour weighted by the specific humidity of the same model level $q^{(i)}$:
\begin{equation}
\label{eq:molar_mass}
M^{(i)}=M_\text{d}\cdot \left(1-q^{(i)}\right)+M_\text{v}\cdot q^{(i)},
\end{equation}
where $M_\text{d}$=0.0289652 kg/mol and $M_\text{v}$=0.018016 kg/mol are the molar mass of dry air and water vapour, respectively.

The air density $\rho^{(i)}$ at the $i$th model level was calculated based on the Ideal Gas Law by treating the atmosphere as a mixture of dry air and water vapour:
\begin{equation}
\label{eq:density}
\rho^{(i)} = \dfrac{p_\text{d}^{(i)}\cdot M_\text{d} + p_\text{v}^{(i)}\cdot M_\text{v}}{R\cdot T^{(i)}},
\end{equation}
where $p_\text{d}^{(i)}$ and $p_\text{v}^{(i)}$ are the partial pressure of dry air and water vapour, respectively, at the $i$th model level. The water vapour pressure $p_\text{v}^{(i)}$ was calculated as \cite{murray1967computation,shaman2009absolute}:
\begin{equation}
\label{eq:pressure_water_vapour}
p_\text{v}^{(i)}=\dfrac{q^{(i)}\cdot p^{(i)}}{\dfrac{M_\text{v}}{M_\text{d}} + \left(1-\dfrac{M_\text{v}}{M_\text{d}} \right)\cdot q^{(i)}},
\end{equation}
where $p^{(i)}$ is air pressure and $q^{(i)}$ is specific humidity at the $i$th model level, both of which were provided by CAMS EAC4. Given $p_\text{v}^{(i)}$, the dry air pressure $p_\text{d}^{(i)}$ can be calculated as:
\begin{equation}
\label{eq:pressure_dry_air}
p_\text{d}^{(i)}=p^{(i)}-p_\text{v}^{(i)}.
\end{equation}

Nitrogen ($N_2$), oxygen ($O_2$), and carbon dioxide ($CO_2$) constitute 75.523\%, 23.133\%, and 0.053\%, respectively, of dry air by mass ratio (\emph{i.e.}, in unit of kg/kg). Although the compositions of these gasses in dry air don't change with altitude, their compositions in total air do due to the vertical variations of water vapour content. To this end, the nitrogen concentration $N_2^{(i)}$ (in unit of kg/kg), oxygen concentration $O_2^{(i)}$ (in unit of kg/kg), and carbon dioxide concentration $CO_2^{(i)}$ (in unit of kg/kg) at the $i$th model level were calculated with the specific humidity of that model level $q^{(i)}$ being considered:
% \begin{equation}
% \label{eq:nitrogen}
% N_2^{(i)}=\left(1-q^{(i)}\right)\times 0.75523,
% \end{equation}
% \begin{equation}
% \label{eq:oxygen}
% O_2^{(i)}=\left(1-q^{(i)}\right)\times 0.23133,
% \end{equation}
% \begin{equation}
% \label{eq:carbon_dioxide}
% CO_2^{(i)}=\left(1-q^{(i)}\right)\times 0.00053,
% \end{equation}
\begin{align}
\label{eq:nitrogen}
N_2^{(i)} &= \left(1 - q^{(i)}\right) \times 0.75523, \\
\label{eq:oxygen}
O_2^{(i)} &= \left(1 - q^{(i)}\right) \times 0.23133, \\
\label{eq:carbon_dioxide}
CO_2^{(i)} &= \left(1 - q^{(i)}\right) \times 0.00053,
\end{align}
